Temporal-Logic-Based Reward Shaping for Continuing Reinforcement Learning Tasks

In continuing tasks, average-reward reinforcement learning may be a more appropriate problem formulation than the more common discounted reward formulation. As usual, learning an optimal policy in this setting typically requires a large amount of training experiences. Reward shaping is a common approach for incorporating domain knowledge into reinforcement learning in order to speed up convergence to an optimal policy. However, to the best of our knowledge, the theoretical properties of reward shaping have thus far only been established in the discounted setting. This paper presents the first reward shaping framework for average-reward learning and proves that, under standard assumptions, the optimal policy under the original reward function can be recovered. In order to avoid the need for manual construction of the shaping function, we introduce a method for utilizing domain knowledge expressed as a temporal logic formula. The formula is automatically translated to a shaping function that provides additional reward throughout the learning process. We evaluate the proposed method on three continuing tasks. In all cases, shaping speeds up the average-reward learning rate without any reduction in the performance of the learned policy compared to relevant baselines.

==> 4_synthesis.tex <==
\section{Potential Function Synthesis}
In this section we present an algorithm for constructing a potential function $\Phi$ from a given temporal logic specification $\varphi$. 
%\commentp{We do need some text here}

\subsection{Safety Game} 
Informally, the reward shaping function captures the information of a safety formula $\varphi$ by \emph{penalizing} the learning agent when it violates $\varphi$. Hence, we introduce a \emph{monitor} that keeps track of the learning agent's behaviour with respect to $\varphi$. We model the interaction between the learning agent and the monitor as a 2-player game between an environment and a controller. The learning agent (environment) chooses an input by taking an action. The monitor (controller) observes this input and chooses an output. The two players then jointly transition and the process repeats. 

A \emph{\textbf{game structure}} is a tuple 
$\game = (\gstates, \ginit, \ialphabet,\oalphabet T,\Acc)$,
where $\gstates$ is a finite set of states, $\ginit \in \gstates$ the initial state,
 $\ialphabet$ and $\oalphabet$ are the alphabet of actions available to the environment and the controller respectively, 
 $T: \gstates \times \alphabet \rightarrow \gstates$
is a complete transition function, that maps each state, input and output to a successor state and
 $\Acc: \left(\states \times \alphabet \times \states\right)^\omega \rightarrow \mathbb{B}$ is the \emph{winning condition} of the game. A \emph{safety game} is a class of game structure where the winning condition $\Acc$ is defined as a set of states $H^g \subseteq G$. A policy for the controller is a mapping $\pi^\mathcal{G}:\gstates \times \ialphabet \rightarrow \oalphabet$. A policy is winning if it induces a winning play. The \emph{winning region} $\mathcal W \subseteq F^g$ is the set of states from which a winning policy exists. 
% \item $\mathcal L:\gstates
% \rightarrow \ialphabet \times \oalphabet$ is the labeling
% function.


% At every state $\gstate \in \gstates$ (starting with
% $\ginit$), the environment chooses an input $\isymb \in
% \ialphabet$, and then the controller chooses some output $\osymb
% \in \oalphabet$. These choices define the next state $\gstate' =
% \delta(\gstate,(\isymb, \osymb))$, and the process then continues from $\gstate'$. This order of moves
% ensures that at each step the controller's action reacts to the \emph{current}
% action of the environment. The resulting
% (infinite) sequence $\pi = (\gstate_0,\symb_{\inp,0},
% \symb_{\out,0}, \gstate_1) (\gstate_1,\symb_{\inp,1},
% \symb_{\out,1}, \gstate_2) \ldots$ is
% called a \emph{play}, where $\gstate_0$ is the initial state, and for every $i \geq 0$ we have that $\gstate_{i+1} = \delta(\gstate_i,\symb_{\inp,i},\symb_{\out,i})$.  A play $\pi$ is \emph{winning} if $\Acc(\pi) = \top$. A \textbf{\emph{safety game}} is a class of game structure where the winning condition $\Acc$ is defined as a set of states $H \subseteq G$ given by a safety automaton $\varphi$. A play $\pi$ is winning in a safety game if all states $\gstate_i \in H$ for all $i\geq 0$. A strategy for the controller is a mapping $\rho:\gstates \times \ialphabet \rightarrow \oalphabet$. A strategy is winning if it induces a winning play. The winning region $\mathcal W \subseteq H$ is the set of states from which a winning strategy exists. 

% The goal of shielded reinforcement learning is to \emph{synthesize} a reactive system that enforces winning with respect to a safety specification. Typically, the synthesis problem is framed as a finding a winning strategy in a safety game~\cite{bloemshield}. The shield implements the strategy $\rho$ as a reactive system $\shield = (\gstates,\gstate_0,\alphabet,\delta,\rho)$. We refer to this shield as a \emph{hard shield}. The hard shield overwrites the action taken by the agent in order to satisfy the safety specification. In this paper, we generate a \emph{soft shield}, that allows the agent to take the action, but will assign a reward or punishment based on satisfaction of the specification. Informally, we use the hard shield to generate a shaping reward function that we provide to the learning agent on top of its environment reward signal to encourage it to learn faster. 

The true power of this approach is the ability to ``plan ahead''. We illustrate this concept with an example.

\begin{example}
Consider again the example of the service robot tasked with cleaning. Suppose, we wish to provide it with the domain knowledge ``the presence of humans tends to increase trash production.'' We can provide this knowledge in the form of an LTL formula ``Always maintain vision of humans.'' Formally, this knowledge will be provided as a safety automaton with a set of safe states $H$ that includes all joint states of the robot and any humans such that the humans are always in vision. However, in order to always not\commentp{never?} violate this safety formula, the robot must ``plan ahead'' to ensure that no matter what the human does in the future the robot will still not lose them. \suda{maybe also cut for space}
\end{example}

The above example illustrates the non-trivial nature of designing shaping functions. It is not enough to penalize just states that are violating the safety formula, but the shaping function must also penalize states from which the \emph{safety formula can be violated in the future}. 

\subsection{Deterministic abstraction}
We introduce a deterministic abstraction of an MDP $\mathcal{M}$ with respect to safety formula $\varphi$. There are two main reasons for using an abstraction. Firstly, the original MDP may have a large number of states which the monitor does not need to distinguish in order to track satisfaction $\varphi$. For example, if the specification is `always stay in the kitchen', there is no need to distinguish between individual states in a bedroom. Second, we can abstract away the stochasticity of the MDP allowing us to use efficient off-the-shelf reactive synthesis tools to solve the resulting safety game. 

% Given an MDP $\mathcal{M} = (\mathcal{S},s_{I}\mathcal{A},R,P) $, labelling function $L$, and automaton $\aut^{\varphi} = (\states,\state_0,2^{\AP},\delta,F)$ and $\mathcal{M}$, a deterministic abstraction of $\mathcal{M}$ with respect to $\varphi$ is $\mathcal{M}^{\varphi} = (S^{\varphi},s_I^{\varphi},\mathcal{A}^{\varphi},\Delta)$ where $\mathcal{A}^{\varphi} = \mathcal{A} \times 2^{\AP}$, $\Delta(s^{\varphi}_{i},a^{\varphi}_i) = \delta(s^{\varphi},L(s_i)$

 A \emph{deterministic abstraction} of MDP $\mathcal{M} = (\mathcal{S},s_{I},\mathcal{A},R,P) $, with respect to automaton $\aut^{\varphi} = (\states,\state_I,2^{\AP},\delta,H)$ is defined as $\aut^{\varphi}_{\mathcal{M}} = (Q^{\mathcal{M}},q_I^{\mathcal{M}},\mathcal{A}^{\varphi}_\mathcal{M},\Delta,H)$ where  $\mathcal{A}^{\varphi} = \mathcal{A} \times 2^{\AP}$ and $\Delta: A \times 2^{\AP} \rightarrow Q^{\mathcal{M}}$. $\aut^{\varphi}_{\mathcal{M}}$ is \emph{sound} if and only if a trace $\sigma = s_0s_1\dots \in \mathcal S^\omega$ with corresponding action sequence $a_0a_1\dots \in \mathcal{A}^\omega$ and word $L_{\varphi}(\sigma)=w_0w_1\dots \in (2^\AP)^{\omega}$ induces a run such that $q_i^{\mathcal{M}} \in H$ for all $i \geq 0$ implies $q_i \in H$ for all $i \geq 0$. Informally the abstraction is sound if a trace in $\mathcal{M}$ induces a satisfying run in $\aut^{\mathcal{M}}_{\varphi}$ then it must also induce a satisfying run in $\aut_{\varphi}$. Note that the converse is not necessarily true. Hence the abstraction is conservative. 

% \begin{figure}
%     \centering
%     \input{figures/cleaning_example_abstraction}
%     \caption{Caption}
%     \label{fig:my_label}
% \end{figure}

% \begin{example}
% \suda{Need to give example of an abstraction here. } No space
% \end{example}

\subsection{Potential Function Synthesis}

Given an average-reward RL problem where an agent has to learn an optimal policy in MDP $\mathcal{M} =\left(\mathcal{S},s_I,A,R,P\right)$, a safety formula $\varphi$. 


 \begin{enumerate}
     \item Construct safety game $\game = (\gstates, \ginit, \ialphabet,\oalphabet, T,H^g)$  from safety automaton $\aut^{\varphi} = (\states,\state_0,2^{\AP},\delta,H)$ and sound deterministic abstraction $\aut^\mathcal{M}$. We construct the game as follows : $\gstates = \states^{\mathcal{M}}\times \states $,  $\ginit = (\state_I^\mathcal{M},\state_I)$, $\ialphabet = \mathcal{A}\times 2^{\AP}$, $\oalphabet = \mathcal A$,      $T((\state^{\mathcal{M}},\state),(a_\inp,L(s)),a_\out) = (\Delta(a_\inp,L(s)),\delta(q,L(s)))$ , 
          $H^g = (\states^\mathcal{M}\times H) $. 

     
     \item Solve the game and compute the winning region $\mathcal{W} \subseteq H^g$ using standard techniques shown in~\citep{bloem2015shield}. 
     \item Recall that the monitor acts as the output in the game. Hence, we use the actions of the monitor to construct $\Phi$ as follows:
     \begin{equation}
         \Phi(s,a) = \begin{cases}
         C & \pi^\mathcal{G}(q^{\mathcal{M}},q,a) = a \\
         d(s) & (\Delta(a,L(s)),\delta(q,L(s))) \notin \mathcal{W} 
         \end{cases}
     \end{equation}
     where $d(s)$ is a \emph{distance} metric to the set $\mathcal{W}$ and $C \in \mathbb{R}$ is a scalar constant.  
     \end{enumerate}
\suda{Resolve consistency issues with s and q - how to define potential function on an mdp that depends on states of automaton?}
%  \begin{example}
%  \suda{Continue running example here}. No space??. 
%  \end{example}




==> problem_statement.tex <==
\section{Problem Statement}
The objective of this paper is to provide shaping rewards for the average-reward setting in reinforcement learning, based on LTL specifications from domain experts. The additional rewards should guide the learning agent towards policies that satisfy the specifications, and thus speed up the learning rate, %but do not prevent learning the optimal policy if it violates the specification. Formally,
%that the optimal policy $\pi^*_\mathcal{M}$ likely statisfies, how to use the specification to guide an average-reward reinforcement learning agent, while allowing $\pi^*_\mathcal{M}$ to be learned even if it violates $\varphi$.

\paragraph{Problem 1:}
Given an MDP $\mathcal{M} = (S,s_I,\mathcal{A},R,P)$ with unknown $R$ and a LTL safety formula $\varphi$ design function $F$ such that, $\pi_{\mathcal{M}}^\ast$ can be learned in MDP $\mathcal{M}' = (S,s_I,\mathcal{A},R+F,P)$ even if it has to violate $\varphi$.


%  

==> supplementary_material/experiment.tex <==
\section*{Gridworld Experiments}

\begin{figure}[h!]
    \centering
     \input{figures/simple_gridworld}
%     \subfloat[Domain knowledge DFA]{\begin{tikzpicture}
% 		\node[state, initial left]  (q0) {$q_I$};
% 			\node[state,accepting] [above right= 0.15cm and 1 cm of q0] (q1) {$q_1$};
% 			\node[state] [below right= 0.15 and 1 cm of q0] (q2) {$q_2$};
% % 			\node[state, accepting] [right=of q1] (q3) {$q_3$};
% % 			\node[state] [right=of q2] (q4) {$q_4$};
% 			\draw 
% 			[->] (q0) edge node[above, sloped] {\tiny$\lnot G$} (q2)
% % 			(q0) edge[bend right=80] node[below, sloped] {\tiny$cr \wedge ! (g1 \wedge g2)$} (q4)
% 			(q0) edge node[above, sloped] {\tiny $G$} (q1)
% 			(q1) edge node[right] {\tiny $\lnot G$} (q2)
% 			(q1) edge[loop right] node[right] {\tiny $G$} (q1)
% 			(q2) edge[loop right] node[right] {\tiny $\lnot G$} (q2);

			
% \end{tikzpicture}}
    \caption{Variations on the grid world case study from~\cite{mahadevan1996average}. Agent receives a reward when it moves to the green cell and is then transported to a random cell.}
    \label{fig:gridworld_setup}
\end{figure}

We evaluate our method against standard R-Learning in a continuing grid world environment as studied by~\cite{mahadevan1996average}. Figure~\ref{fig:gridworld_setup} shows the 6*6 grid with a +100 reward in the green cell. The agent can move to a neighboring cell in one of the four directions deterministically at every step, and gets ``transported'' to a random cell when it reaches the green cell and when it fails to reach the green cell after 100 steps. %The purpose of this experiment to showcase that our temporal-logic-based reward shaping approach is able to increase learning rate even when the environment is different to what was initially given. In this experiment, we compute the reward shaping function for the grid world without a wall as shown on the left in Figure 1, and compare the rate of learning when there is an unexpected wall in the grid world as shown on the right. 

The following four methods are compared: our temporal-logic-based reward shaping, hand-crafted reward shaping~\citep{ng1999policy}, shielding, and baseline R-learning. Shielding blocks actions up and left and only allows actions down and right. For the temporal-logic-based method, the winning region consists of all states, but only with the actions down and right. Then the potential function $\Phi$ is constructed with $C=1$ and $d(s,a)=-1$. The hand-crafted potential function is taken from the grid world experiments by~\cite{ng1999policy}, where $\Phi(s)$ is defined as the negative of the distance from $s$ to the green cell.
%\suda{I think we remove the state based shaping, it's not necessary and doesn't add to the message} \commenty{The original reward shaping paper had this experiment, so it makes sense to show our shaping function is no worse than the original one.}
%\commenty{Describe temporal logic in notations defined in Sec. 4. Summarize learning parameters.}

The correctness of the advice is varied by adding the wall from (2, 2) to (2, 5) as shown in Figure~\ref{fig:gridworld_setup}. When the agent is directly above the wall, it cannot reach the green cell by only moving down or right. This experiment evaluates our temporal-logic-based reward shaping framework when the environment is different from what the advice is given for.%\suda{Does the actual reward move or does our knowledge move?}
%We conduct experiments in four conditions: no wall and correct position, no wall and wrong position, with wall and correct position, and with wall and wrong position. 

\begin{figure*}[h!]
    \centering
    \subfloat[Perfect knowledge.]{\input{figures/gridworld_simple}}
    \centering
    \subfloat[Unexpected wall.]{\input{figures/gridworld_wall}}
    
    %\centering
    %\subfloat[Imperfect knowledge about goal.]{\input{figures/gridworld_wrong_goal}}
    %\centering
    %\subfloat[Imperfect knowledge about wall and goal.]{\input{figures/gridworld_wrong_goal_and_wall}}
    \caption{Learning performance comparison of temporal-logic-based reward shaping (ours), hand-crafted reward shaping (Ng et al.), shielding, and baseline. The average reward of every 100 steps is plotted, averaged by 100 runs. }
    \label{fig:gridworld}
\end{figure*}

Figure~\ref{fig:gridworld} compares the learning performance of each method in the two conditions. The observations are consistent with the results reported in other benchmarks in the paper. Shielding outperforms other methods when the advice is perfect, i.e., there is no wall, and fails to reach the maximum average reward when the wall is added. Our temporal-logic-based reward shaping method performs similarly to the hand-crafted shaping function while allowing the reward shaping to be automatically constructed. Both shaping methods still outperform the R-learning baseline when the advice is imperfect. 

